Out-of-Vocabulary Challenge Report

This paper presents final results of the Out-Of-Vocabulary 2022 (OOV) challenge. The OOV contest introduces an important aspect that is not commonly studied by Optical Character Recognition (OCR) models, namely, the recognition of unseen scene text instances at training time. The competition compiles a collection of public scene text datasets comprising of 326,385 images with 4,864,405 scene text instances, thus covering a wide range of data distributions. A new and independent validation and test set is formed with scene text instances that are out of vocabulary at training time. The competition was structured in two tasks, end-to-end and cropped scene text recognition respectively. A thorough analysis of results from baselines and different participants is presented. Interestingly, current state-of-the-art models show a significant performance gap under the newly studied setting. We conclude that the OOV dataset proposed in this challenge will be an essential area to be explored in order to develop scene text models that achieve more robust and generalized predictions.

==> sota/sota.tex <==
Scene text detection and recognition is a challenging topic that has been an active area of research for many years. The complexity and sophistication of the architectures increased as different datasets and annotation styles started emerging. The simplest scenario for text detection features horizontal bounding boxes \cite{karatzas2013icdar}, incidental text with 4-point annotations \cite{karatzas2015icdar, nayef2017icdar2017, singh2021textocr, veit2016coco} and more recently arbitrarily shaped text \cite{ch2017total, liu2019curved} such as curved text, which often contain complex polygonal annotations.

The first deep learning approaches towards scene text understanding separated the detection and the recognition in two separate steps, a detection and a recognition network. The most commonly used recognition architectures, such as the encoder-decoder \cite {lee2016recursive, cheng2017focusing} or the CTC-based \cite {graves2006connectionist} networks, require the text to be horizontal and from left to right. Simpler models such as Textboxes \cite{liao2017textboxes} directly cropped the detected horizontal boxes from the image, and performed no rectification to the crop. As the complexity of annotations increased, models started to feature two-stage architectures that were fully end-to-end trainable and perform complex RoI rectifications to the detected areas. For example, FOTS \cite{liu2018fots} features a end-to-end trainable two-stage architecture that is capable of detecting and rectifying rotated bounding boxes. More complex architectures, such as ABCNet \cite{liu2020abcnet} or TextDragon \cite{feng2019textdragon}, started taking advantage of complex polygonal annotations to better rectify the text.


%\subsection{Text Recognition}

In text recognition, cropped word instances are presented to a recognition network, which generates sequences of characters. This area has traditionally been dominated by two approaches, encoder-decoder\cite{sutskever2014sequence} networks and CTC-based\cite{graves2006connectionist} decoders. These two approaches process sequences of 1-dimensional data to generate outputs of the same shape, making them suitable to text recognition. Recognition architectures employ CNNs to encode the image into sequences of features, which are then fed to the decoder. DTRN\cite{he2016reading} was the first model that used a CTC-based decoder. The authors generate convolutional feature slices using a convolutional recurrent neural network (CRNN), which are then fed to a RNN (where the CTC loss is used to learn the representation). In encoder-decoder networks (such as \cite{lee2016recursive, cheng2017focusing}), the visual features are encoded into a latent representation and then decoded into a character sequence. In both approaches the encoded image has to be fed sequentially (usually from left to right), which requires the text to be presented horizontally. This is particularly a problem for scene text detection and recognition architectures that use these techniques, since many datasets feature oriented and curved text instances.

In the literature we can find other approaches to text recognition that do not employ CTC or encoder-decoder networks. For example, Jaderberg et al.\cite{jaderberg2016reading} treat the scene-text recognition problem as a classification problem. A convolutional network classifies each cropped word into different classes, where each class belongs to a different word of a large dictionary. The biggest drawback of this approach is that out-of-dictionary words cannot be recognized. Gomez et al.\cite{gomez2018cutting} use a similar convolutional network to read utility meters, in this case each number of the meter is treated as a classification problem. More recently, a vision transformer-based model\cite{atienza2021vision} uses a transformer encoder to perform text recognition. The author inputs embedded crops of the image jointly with learnable classification tokens to the encoder, where the word recognition is embedded.

% scatter and other such approaches are missing

\subsection{Two-Stage Methods}

Two-stage architectures feature end-to-end trainable networks, benefiting from shared features and common gradient flow. Different methods of RoI cropping and pooling allow recognition of text in different shapes and orientations. However, these methods still treat detection and recognition as separate tasks, with the recognition stage heavily depending on the detections and the RoI methods. For example, FOTS \cite{liu2018fots} uses a text detection branch to predict oriented text boxes, and uses RoIRotation to obtain axis-aligned feature maps. The text recognition branch uses a bidirectional LSTM \cite{schuster1997bidirectional, hochreiter1997long} and then uses a CTC \cite{graves2006connectionist} network to recognize the crop.
%He et al.\cite{he2018end} adopt the Mask-RCNN architecture to generate the proposals and RoIAlign\cite{he2017mask} to correct the detected text before passing it to an LSTM with attention. Another effective way of dealing with distorted text is using segmentation networks\cite{lyu2018mask, liao2020mask}.
Mask TextSpotterV3 \cite{liao2020mask} extracts rectangular crops from the segmentation and then masks-out the area outside of the region of interest. ABCNet \cite{liu2020abcnet} uses a more unconventional approach by fitting Bezier curves to the text instances, which helps obtaining smoother boundaries around the words. The curves are rectified with their proposed BezierAlign, which uses the control points of the curves to warp the word into a rectangular shape.
%Wang et al.\cite{wang2020all} generate oriented bounding boxes and use two RoI operations to rectify the detections, first a RoIRotation to axis-align the box and then an arbitrary RoI align to finally adjust arbitrarily distorted text. 
TextDragon \cite{feng2019textdragon} predicts a series of quadrangles that follow the shape of the words and use their own RoISlide to rectify the text. 

Many of the previous corrective RoI methods (such as the masking approaches) require polygonal contours that are more expensive to annotate. The currently largest scene-text datasets feature oriented quadrilaterals \cite{singh2021textocr} or axis-aligned \cite{veit2016coco} annotations, making some of the previous approaches difficult to use in such scenarios.


\subsection{One-Stage Methods}

More recently, one-stage methods have started appearing and have shown success on different benchmarks. These approaches diminish the dependence between the detection and recognition stages, and avoid relying on complex RoI operations. The authors of \cite{gomez2018single} present one of the first attempts at a single stage architecture, in this case for scene text retrieval. The authors predict the location and PHOC \cite{almazan2014word} representation of each word in the scene using a YOLOv2\cite{redmon2017yolo9000} architecture. The first single-stage architecture for text detection and open recognition was by Xing et al. \cite{xing2019convolutional}, where a convolutional network outputs bounding boxes at character-level with the corresponding character label. MANGO \cite{qiao2020mango} is another example of one-stage architecture, where the outputs of a FPN \cite{lin2017feature} are fed into a mask attention module, followed by a recognizer that outputs character sequences in each cell of a grid.

% transformer-based methods
A common trend is to use transformer-based~\cite{vaswani2017attention} networks that exploit the self attention mechanism to avoid complex RoI rectifying operations, and some of them are even capable of using simple annotations such as central keypoints.
For example, in TTS \cite{kittenplon2022towards}, a shared transformer encoder-decoder is used by different heads to perform word recognition, detection and segmentation. This method can be trained by either providing the polygon annotations, the bounding box, or only the text. Finally, in SPTS \cite{peng2021spts} the authors use a transformer encoder-decoder network to predict point coordinates and text transcriptions. \cite{peng2021spts, zhang2022text} also employ encoder-decoder approaches to do the text detection and the recognition. More recently, DEER ~\cite{kim2022deer} uses a transformer encoder to perform detection-agnostic detection and recognition. 

%\cite{huang2022swintextspotter} missing but not too interesting
